Boost Video Frame Interpolation via Motion Adaptation

Video frame interpolation (VFI) is a challenging task that aims to generate intermediate frames between two consecutive frames in a video. Existing learning-based VFI methods have achieved great success, but they still suffer from limited generalization ability due to the limited motion distribution of training datasets. In this paper, we propose a novel optimization-based VFI method that can adapt to unseen motions at test time. Our method is based on a cycle-consistency adaptation strategy that leverages the motion characteristics among video frames. We also introduce a lightweight adapter that can be inserted into the motion estimation module of existing pre-trained VFI models to improve the efficiency of adaptation. Extensive experiments on various benchmarks demonstrate that our method can boost the performance of two-frame VFI models, outperforming the existing state-of-the-art methods, even those that use extra input.

==> section/9_limitation.tex <==
\label{limitation}
Our proposed method still has certain limitations: Due to the limitation of data and computing resources, our motion adaptation strategy is currently restricted to 2-frame VFI models and has not been extended to frame synthesis at arbitrary temporal positions. 
Moreover, in general, our proposed method is beneficial for better handling regular motions, such as rotations and large-scale motions, however, it remains challenging for irregular motions, such as sudden camera shaking, or illumination changes, due to the difficulty of inferring priors.
Our future work will investigate more efficient plug-in adapter architecture and further extend it to flexible VFI models with multiple frames as inputs, which has the potential to further boost the performance and generalisation ability of video frame interpolation models.

==> table/table0_archived.tex <==
\begin{wraptable}{r}{7.8cm}
% \vspace{-.3cm}
\setlength\tabcolsep{8pt}  
\centering
\resizebox{.58\textwidth}{!}{%
\begin{tabular}{cc|cc|cc}
\hline
\multicolumn{2}{c|}{} & \multicolumn{2}{c|}{Direct} &  \multicolumn{2}{c}{Cycle-Consistency} \\ \hline
\ Method \ & \ \#adaptation \ & PSNR & SSIM & PSNR & SSIM \\ \hline
\multirow{3}{*}{IFRNet~\cite{kong2022ifrnet}} 
& 0  & 35.86 & 0.9729 & 35.86 & 0.9729 \\ 
& 5  & 35.95 & 0.9734 & 36.14 & 0.9741 \\ 
& 10 & 35.81 & 0.9731 & 36.38 & 0.9753 \\ \hline
\multirow{3}{*}{UPRNet~\cite{jin2022unified}} 
& 0  & 36.07 & 0.9735 & 36.07 & 0.9735 \\ 
& 5  & 36.23 & 0.9744 & 36.49 & 0.9750 \\ 
& 10 & 36.16 & 0.9747 & 36.68 & 0.9758 \\ \hline
\end{tabular}
}
\vspace{5pt}
\caption{\textbf{Quantitative comparison of Test-time adaptation strategies} on Vimeo90K dataset. Both adaptation strategies are effective, while Cycle-Consistency Adaptation achieves stable performance improvement by leveraging the consistency within the video sequence.}
\label{tab:table1}
\vspace{-5pt}
\end{wraptable}
